UnScene3D: Unsupervised 3D Instance Segmentation for Indoor Scenes

3D instance segmentation is fundamental to geometric understanding of the world around us. Existing methods for instance segmentation of 3D scenes rely on supervision from expensive, manual 3D annotations. We propose UnScene3D, the first fully unsupervised 3D learning approach for class-agnostic 3D instance segmentation of indoor scans. UnScene3D first generates pseudo masks by leveraging self-supervised color and geometry features to find potential object regions. We operate on a basis of geometric oversegmentation, enabling efficient representation and learning on high-resolution 3D data. The coarse proposals are then refined through self-training our model on its predictions. Our approach improves over state-of-the-art unsupervised 3D instance segmentation methods by more than 300% Average Precision score, demonstrating effective instance segmentation even in challenging, cluttered 3D scenes.

==> 3_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}

%We leverage the principle of the normalized cut algorithm~\cite{shi2000normalized_cut} (NCut) to identify potential instances for 3D pseudo masks, lifted to the high-dimensional 3D scenario by using a geometric primitive basis, as discussed in Section~\ref{sec:oversegmentation}.
\NEW{We employ the principle of the NCut approach for pseudo-generation similarly to \cite{wang2023cut}, but lift it to support high-resolution 3D segmentation by operating on segment-level geometric primitives from self-supervised 2D and 3D features.}

NCut maximizes similarities within partitions and dissimilarities across partitions by minimizing the cost of a graph cut. This is formalized as: 
%
\begin{equation}
    NCut(A,B) = \frac{cut(A,B)}{assoc(A,V)} + \frac{cut(A,B)}{assoc(B,V)},
\end{equation}
where $A$ and $B$ are disjoint bipartitions from a full graph $V$, $cut$ measures the degree of dissimilarity computed as the total weight of edges that have been removed, and  $assoc$ represents the total connection within the partition.
Normalizing the cut cost function with the size of the partitions can solve the problem of single outlier node removal, which is one of the biggest difficulties of other graph cut algorithms~\cite{244673}.

While the minimum solution of this problem is intractable for practical applications, it can be rewritten as a generalized eigenvalue problem with adjacency matrix $W$ and degree matrix $D$, where $D(i,i) = \Sigma_jW(i,j)$:
%
\begin{equation} \label{eq:general_eigenval}
    (D-W)v = \lambda D v,
\end{equation}
%
Finding the second smallest eigenvalue $\lambda$  and its corresponding eigenvector $v$ is a close approximation for the minimized cost. 
From $v$, we obtain foreground separation by taking all node activations where the eigenvector components were larger than their mean. 
This method has been shown to be effective on intensity images, but combining it with deep features has demonstrated even stronger potential in the image domain \cite{wang2022tokencut,lis2022attentropy,wang2023cut}. 
While this multiple foreground objects could be directly predicted with a single pass by taking the eigenvectors in order, it was shown in \cite{wang2022tokencut} that a greedy iterative approach produces better results.




